WISE: Unraveling Business Process Metrics with Domain Knowledge

Anomalies in complex industrial processes are often obscured by high variability and complexity of event data, which hinders their identification and interpretation using process mining. To address this problem, we introduce WISE (Weighted Insights for Evaluating Efficiency), a novel method for analyzing business process metrics through the integration of domain knowledge, process mining, and machine learning. The methodology involves defining business goals and establishing Process Norms with weighted constraints at the activity level, incorporating input from domain experts and process analysts. Individual process instances are scored based on these constraints, and the scores are normalized to identify features impacting process goals. Evaluation using the BPIC 2019 dataset and real industrial contexts demonstrates that WISE enhances automation in business process analysis and effectively detects deviations from desired process flows. While LLMs support the analysis, the inclusion of domain experts ensures the accuracy and relevance of the findings.

==> Chapters_Singular/1_Introduction.tex <==

\section{Introduction}
Process mining techniques primarily aim to discover, monitor, and enhance real-world processes by extracting valuable knowledge from event logs within organizational information systems \cite{van2012process}. In industrial contexts, companies utilize process mining to achieve business goals such as improving process efficiency or reducing process costs \cite{reinkemeyer2020process}. However, the complexity of processes with numerous variants, coupled with broad contextual data and the fact that non-technical experts are often the ultimate recipients, makes these projects challenging for many companies \cite{grisold2021adoption, eggert2022applying, badakhshan2022creating}.

Our method, WISE (Weighted Insights for Evaluating Efficiency), aims to address these challenges by facilitating faster and more interpretable insights from process analysis. WISE combines domain knowledge, process mining, and machine learning techniques to provide a comprehensive methodology for analyzing business processes. This methodology enables the identification of process inefficiencies and anomalies by understanding the impact of various features or dimensions on process outcomes. By focusing on approximation and summarization, WISE aims to distinguish between 'process noise' and actionable insights, thereby enhancing decision-making for non-technical experts.

Process analysis involves examining and evaluating the various steps and activities within a process to identify inefficiencies, bottlenecks, and areas for improvement \cite{taymouri2021business}. In both academia and industry, there is growing interest in utilizing different algorithms and tools to support process analysis \cite{marcelo2016process}. Over the last decade, process mining has developed a set of tools for process analysts, ranging from process discovery to process enhancement and conformance algorithms \cite{van2022process}. However, most methods examine processes primarily from a process flow perspective \cite{van2022process}, without considering additional contextual data or domain knowledge, focusing mainly on the main behavior. Additionally, there remains a gap in academic research in applying process mining in complex scenarios \cite{taymouri2021business, thiede2018process} and improving understandability for non-experts \cite{thiede2018process}.


At the same time, software vendors offer a plethora of templates, apps, and dashboards addressing various types of processes and business problems. For example, as of this publication, Celonis—one of the market leaders in process mining—offers over 145 different apps in their marketplace for procurement alone, each containing dozens of dashboards, KPIs, and tables. These are often connected to hundreds of tables in enterprise systems, adding an additional layer of complexity. Due to the vast number of features and combinations, significant time and expertise are required to sift through the data to find what is relevant. Additionally, most steps of analyzing the root causes for discovered inefficiencies are performed manually.

In this paper, we address the following problem: Event logs typically used in industry contain not only different process flow variants but also many features and attributes. Process instances executed in a business context can exhibit different performance dependent on different performance criteria. For example, some process instances may be efficient but at the same time costly due to extensive manual labor. Our method aims to (semi-)automatically identify the instances of the process with the highest inefficiencies or outliers, additionally identifying the set of context/data features that summarized explain this impact. Finally, the root causes of the problems can be identified (e.g., vendors, products, variants of the process), which can be addressed with actionable insights—such as renegotiating contracts with specific suppliers, providing training for specific departments, or reengineering parts of the process in specific cases.
\begin{figure}[ht]
  \centering
  \includegraphics[width=\columnwidth]{pictures/Method_WISE_1.png}
  \caption{General WISE Methodology and its main steps.} 
  \label{fig:GeneralMethodology}
\end{figure}


Figure \ref{fig:GeneralMethodology} depicts general steps used in WISE methodology:
\begin{enumerate}
    \item \textbf{Defining Business Goals}: The first step involves defining the business goals, such as reducing costs, increasing automation, and reducing lead times. This sets the context and objectives for the subsequent analysis.
    \item \textbf{Defining Constraints and Weights}: Next, domain experts and/or machine learning models (LLM) collaborate to define constraints and assign weights to each constraint. These constraints are critical in shaping the analysis and ensuring that the most relevant factors are considered.
    \item \textbf{Applying WISE for Analysis}: Using the WISE framework, we apply algorithms to the event logs to find anomalies and deviations in different dimensions. This involves comparing all traces to the intended flow and computing deviation statistics against each feature-value combination.Each process instance is evaluated and scored based on constraints and weights for each of previously defined objectives. 
    \item \textbf{Visualization and Insight Generation}: The deviation analysis is visualized at a fine-grained level to reveal the exact features contributing to specific performance deviations. The individual process instances scores are aggregated for different dimensions. This helps in identifying the root causes of inefficiencies and generating actionable insights.
    \item \textbf{Actionable Insights for Improvement}: Finally, the insights derived from the analysis are used to address the identified issues. For example, this could involve renegotiating contracts with specific suppliers, providing targeted training for departments, or reengineering parts of the process.
\end{enumerate}
This methodology aims to simplify the assessment of business process indicators by making them more interpretable and actionable for professionals through simplification and approximation. By utilizing specialized industry knowledge and focusing on essential tasks, we intend to clarify these indicators for different stakeholders in process mining projects.


The remainder of this paper includes a problem description, methodology discussion, and evaluation results using the BPI 2019 dataset. We also report on applying the method to industrial case study summarizing feedback from process owners, who indicated that the method effectively identified actionable issues.










==> Chapters_Singular/2_Related_Work_Problem_Desc.tex <==
\section{Related Work and Problem Description}
The need for process improvement has been a critical focus for organizations striving to enhance operational efficiency and effectiveness. Historically, businesses have continuously sought methods to refine their internal processes to achieve these goals. Business Process Analysis (BPA) emerged as a foundational approach to systematically examine and improve business processes\cite{dumas2018introduction}.Traditionally, BPA methods have been time-consuming, involving extensive meetings, document analysis, and direct observation. These traditional methods often lead to discrepancies between actual and perceived processes, particularly in complex scenarios \cite{stefanini2020process}.

Process mining has evolved as a semi-automated approach to BPA, leveraging data from software systems to discover, check conformance, and enhance processes \cite{van2012process}. 
Process Mining Research has been striving to support industry in analyzing real life processes by developing different algorithms and methods.Key techniques used in process mining for analyzing complex process environments include among others:
\begin{enumerate}
    \item \textbf{Procedural Process Mining}: Algorithms such as Fuzzy Mining and clustering techniques simplify complex models, making them more understandable and manageable.
    \item \textbf{Declarative Process Mining}: Utilizing constraint-based languages to define flexible sequences of activities, allowing for more adaptive and resilient process designs \cite{stefanini2020process}.
\end{enumerate}

Despite those advancements in process mining, significant challenges remain unresolved. The Process Mining Manifesto \cite{van2012process} outlines 11 broad challenges, including dealing with complex event logs and improving understandability for non-experts. Also many publications identify challenges such as managing complex business processes and \cite{eggert2022applying}, securing stakeholder buy-in, and aligning expectations\cite{dakic2019process} as critical for effective process mining adoption.Similarly R’Bigui and Cho \cite{r2017state} and Munoz-Gama et al. \cite{munoz2022process} note that many of these challenges remain unresolved.Additionally Thiede et al. emphasize the need for more research on applying process mining in complex scenarios \cite{thiede2018process}.


\begin{figure}[ht]
  \centering
  \includegraphics[width=\columnwidth]{pictures/Outlier_Types.png}
  \caption{Structural and contextual outliers. Based on \cite{liu2022benchmarking}, modified.} 
  \label{fig:ContextualOutlier}
\end{figure}

One of the features of such complex, multi-variant processes is the presence of noise, outliers, and infrequent behavior\cite{koschmider2021demystifying}. In event logs, outliers are defined as unusual or exceptional instances that deviate from normal patterns, while noise refers to random or erroneous data points that do not follow expected behaviors \cite{koschmider2021demystifying}. A common technique for simplifying data interpretation is filtering out such instances \cite{van2020detection, sun2019filtering}. However, Koschmider et al. argue that detecting and addressing contextual outliers, which are unusual within specific contexts, and collective outliers, which are subsequences deviating from the norm even if individual activities are typical, is crucial for improving process mining accuracy and gaining valuable process insights \cite{koschmider2021demystifying}. As proposed by Liu et al.\cite{liu2022benchmarking} WISE Methodology uses contextual outliers, calculating scores for event or process instance features as depicted in figure \ref{fig:ContextualOutlier}.

Despite the increase in commercial software tools capable of generating dashboards and visualizations directly from core data systems like SAP, the anticipated business value may not always be achieved, potentially leading to disillusionment \cite{emamjome2019case}. The challenge in process mining involves enhancing output clarity and usability for non-expert stakeholders, especially within complex industrial settings \cite{van2012process}. Transforming complex data into understandable insights remains a well-known issue in data science, highlighting the importance of 'analytics translators'—professionals skilled at interpreting data to identify business challenges and convert needs into data-driven inquiries \cite{herring2019train, zhang2023deliberating}.

Traditional algorithms often produce overly complex, "spaghetti-like" models in unstructured processes, complicating interpretation \cite{stefanini2020process}. Successful process mining projects require methodologies that integrate domain knowledge, set clear process goals, encourage iterative analysis, and provide clear, practical guidelines for each project stage 
 \cite{van2015pm}.

Process mining analysts play a crucial role by obtaining and preparing data, analyzing processes, generating insights, and providing recommendations for improvement \cite{zimmermann2022process}. Zimmerman et al. describes the biggest challenges perceived by process analysts, such as understanding complex process domains and terminology, collaborating with stakeholders, handling the inherent complexity of real-world processes, and ensuring proper training and tool knowledge. These issues underscore the need for better support and solutions to enhance the effectiveness of process mining initiatives \cite{zimmermann2022process, zerbato2021initial, zimmermann2023makes}.

Zimmermann et al. argue that involving stakeholders is a critical strategy to address these challenges. This approach aims to increase understanding, align expectations, and identify key requirements, involving executives, business owners, process owners, IT, and domain experts. Such involvement ensures accurate data interpretation, effective communication, and the development of relevant solutions \cite{zimmermann2023makes}.

The WISE Methodology aims to address described challenges of analyzing processes in complex environments at the same time delivering the interpretable process insights. Using contextual and collective outliers\cite{koschmider2021demystifying} the method on approximation
and summarization to distinguish between mere ’process noise’ and
genuine insights that provide a foundation for actionable decisions. 






==> Chapters_Singular/3_Proposed_Method.tex <==
\section{Proposed Method: WISE}

Our proposed WISE Method is grounded on the business objectives defined by stakeholders, managers and domain experts. 
At the heart of our methodology is the development of a Process Norm. This Norm serves as a reference point, facilitating the distinction between routine data variations—commonly seen as noise—and authentic anomalous activities that merit further analysis for enhanced process understanding. We introduce a quantitative approach that utilizes a weighted scoring system, crafted to assess adherence to these overarching process standards.


The method employs expertise of domain experts in defining process constraints and defining weights for each constraint. This establishes Process Norm which can be further utilised for automated analysis. In absence of domain experts defining constraints and corresponding weights can be also generated automatically through contextualized Large Language Model. Thereafter the WISE algorithms are being applied in order to score each singular instance of process flow, based on established process norm and its deviation from it. Finally the deviations can be calculated based on varying features. In last phase the insights can be derived by process analyst or LLM. If necessary the WISE analysis can be repeated only for selected features and data.

\subsection{Definition of Process Norm}

Initially, we establish the Generalized Process Norm as a comprehensive, multi-layered framework that incorporates essential events and attributes reflective of typical process operations. This norm defines a series of constraints for subsetting the event log, with constraints and weights specified for each business objective, referred to as a view. Each view can be analyzed independently or as part of multiple perspectives on the process. The constraints are organized into different layers, each focusing on a specific aspect:

\begin{itemize}
    \item \textbf{Layer 1}: Mandatory events (without imposing order)
    \item \textbf{Layer 2}: Mandatory ordering of events
    \item \textbf{Layer 3}: Balanced events - events that should occur the same number of times
    \item \textbf{Layer 4}: Singular events - events that should not occur more than once
    \item \textbf{Layer 5}: Exclusive events - events that should not occur at all
\end{itemize}
More layers can be added depending on analysis goals.
This structure allows for a detailed and flexible analysis of business processes according to various objectives.

Process Norms grounds all process instances and enable discovering deviations and inefficiencies in process flow.
We assume as input event log being: event log \(L = (E, \#, \prec)\), where \(E \subseteq U_{\text{ev}}\) represents the set of events, \(\# \in E \rightarrow U_{\text{map}}\) maps events to their attributes, and \(\prec \subseteq E \times E\) establishes a strict partial ordering of events.Additionally 
\[
U_{\text{map}} : U_{\text{attr}} \to U_{\text{val}}
\]

We assume attributes \texttt{activity}, \texttt{case} $\in U_{\text{attr}}$ with their standard interpretation. For a case identifier $c$, the trace is the partial order $\sigma_c \in L = (E_c,\#_c,< _c)$ with events $E_c = \{ e \in E \mid \#_{\text{case}}(e) = c \}$ and $\#_c = \#|_{E_c}$ and $< _c = <|_{E_c \times E_c}$ restricted to $E_c$\cite{van2022process}. From this event log, we identify a subset of events that we call a "Process Norm". For defining this process norm the idea from declarative process modeling languages such as DCR graphs\cite{di2022declarative}, has been simplified  and limited only to most basic constraints as these are easy to understand and specify.


\textbf{Definition (Generalized Process Norm):} A \textit{Generalized Process Norm} \(N\) is defined as a tuple \((C_N, F_N, W_N)\) where:
\begin{itemize}
    \item \(C_N = \{c_1, c_2, \ldots, c_n\}\) represents a predefined set of constraints, each grounded in business understanding.
    \item \(F_N = \{f_1, f_2, \ldots, f_n\}\) denotes a corresponding set of filter functions, where each \(f_i\) applies the constraint \(c_i\) to the event log.
    \item \(W_N = \{w_1, w_2, \ldots, w_n\}\) is a set of weights, where each \(w_i \in [0, 1]\) describes the importance of the constraint \(c_i\) in the overall calculation.
\end{itemize}

Applying the filters \(F_N\) to an event log \(L\) leads to a sublog \(L_N\) containing only the cases that satisfy all the constraints in \(C_N\). The weights \(W_N\) influence the evaluation of the process norm by highlighting the relative importance of each constraint.

--- TODO : IS IT REALLY ? DISCUSS FORMALISATION WITH DIRK

The norm defines six layers of filters:

\begin{enumerate}
    \item \textbf{Layer 1: Foundational Protocols}
        \begin{itemize}
            \item Identify mandatory activities \(M \subseteq U_{\text{attr}}\).
            \item Restrict \(L\) to the subset \(E_M \subseteq E\) of events where \(\#_{\text{activity}}(e) \in M\).
        \end{itemize}
        This layer ensures the presence of essential, predefined events.
        
\textbf{Layer 2: Sequential Directives}

\begin{itemize}
    \item Identify mandatory pairs of activities:
    \[
    <_M \subseteq M \times M
    \]
    This set \( <_M \) contains pairs of activities \((a_1, a_2)\) such that \(a_1\) must eventually be followed by \(a_2\), but not necessarily directly.

    \item Restrict \(L\) to all traces \(\sigma\) where the mandatory sequence is maintained:
    \[
    \forall (a_1, a_2) \in <_M, \exists (e_1, e_2)
    \in <_{\sigma}
    \]
    \[\text{ with } \#_{\text{activity}}(e_1) = a_1, \#_{\text{activity}}(e_2) = a_2, 
    \]
    \[\text{ and } e_1 <_{\sigma} e_2
    \]
    This means for each pair of activities \((a_1, a_2)\) in \( <_M \), there must exist corresponding events \((e_1, e_2)\) in the trace \(\sigma\) such that the activity of \(e_1\) is \(a_1\), the activity of \(e_2\) is \(a_2\), and \(e_1\) happens before \(e_2\) (but they do not have to be directly consecutive).
\end{itemize}

This layer confirms whether specified events occur sequentially, ensuring compliance with essential procedural steps, even if other activities occur in between.

        
\textbf{Layer 3: Equilibrium Standards}

Define harmonization requirements \(H \subseteq E\). This layer ensures the balanced occurrence of specified events.

Formally:
\[
\forall c \in C, \forall h \in H, \text{count}(h, c) = \text{expected}(h)
\]

Where:
\begin{itemize}
    \item \(H = \{h_1, h_2, \ldots, h_k\}\) is the set of events that must be balanced.
    \item \(\text{count}(h, c)\) denotes the number of occurrences of event \(h\) in case \(c\).
    \item \(\text{expected}(h)\) denotes the expected number of occurrences for event \(h\).
\end{itemize}

\textbf{Layer 4: Singularity Criteria}

Identify unique events \(U \subseteq E\) that should not occur more than once in a process instance.

Formally:
\[
\forall c \in C, \forall u \in U, \text{count}(u, c) \leq 1
\]

Where:
\begin{itemize}
    \item \(U = \{u_1, u_2, \ldots, u_m\}\) is the set of unique events.
    \item \(\text{count}(u, c)\) denotes the number of occurrences of event \(u\) in case \(c\).
\end{itemize}

\textbf{Layer 5: Exclusion Guidelines}

Identify undesirable events \(A \subseteq E\) that should not occur at all.

Formally:
\[
\forall c \in C, \forall a \in A, \text{count}(a, c) = 0
\]

Where:
\begin{itemize}
    \item \(A = \{a_1, a_2, \ldots, a_p\}\) is the set of undesirable events.
    \item \(\text{count}(a, c)\) denotes the number of occurrences of event \(a\) in case \(c\).
\end{itemize}

\end{enumerate}
\subsection{Scores Calculation}
Building upon the multi-layered framework for defining process norms, from basic event inclusion to advanced harmonization requirements, we refine the approach for scoring individual process instances. This refined scoring method evaluates the adherence of each process instance to the established norms, encompassing sequence, harmonization, uniqueness, and avoidance norms, thus offering a comprehensive assessment of process conformity.

The traces \( L' \subseteq L \) that are included in the process norm, i.e., those that remain after applying all filters of the process norm, represent all actual process executions that adhere to the process norm. These traces are examples of the preferred way of executing the process as observed in practice.

All other traces, \( L \setminus L' \), deviate from the norm in some manner. However, some deviations result from data variations (i.e., noise) or are harmless (i.e., they show only marginal differences from the norm concerning measures of interest), while other deviating traces are considered anomalies.

---- TODO .... HOW DO YOU FORMAT CORRECTLY

Formally, let:
\[
L' = \{ \sigma \in L \mid \text{trace } \sigma \]
\[\text{ adheres to all constraints in the process norm} \}
\]

\[
L \setminus L' = \{ \sigma \in L \mid \text{trace } \sigma \]
\[\text{ deviates from at least one constraint in the process norm} \}
\]

Where:
\begin{itemize}
    \item \( L \) is the set of all traces in the original event log.
    \item \( L' \subseteq L \) is the subset of traces that adhere to the process norm.
    \item \( L \setminus L' \) is the set of traces that deviate from the process norm.
\end{itemize}

The traces in \( L' \) are considered examples of the preferred way of executing the process. In contrast, the traces in \( L \setminus L' \) include those that are due to noise or marginal differences and those that are considered anomalies.


In order to differentiate marginal differences from actual anomalies (for which the analyst also wants to identify explanations for their occurrence allowing to take action for process improvement) we score individual cases based on their deviations from the norm.


Given:
\begin{itemize}
    \item \textbf{Layer 1: Foundational Protocols} - For the set of all activities \(\Sigma = \{a_1, \ldots, a_n\}\) and a trace \(\sigma_i \in L\) with events \(E_{\sigma_i}\), let \(value_{ij} = |\{ e \in E_{\sigma_i} \mid \#_{\text{activity}}(e) = a_j \}|\) represent the count of how often activity \(a_j\) occurs in \(\sigma_i\).
    
    \item Let \(sum\_counts_i = \sum_{j=1}^{n} value_{ij}\) represent the total count of events for each process instance \(i\), where \(value_{ij}\) is the occurrence count of event \(j\) in process instance \(i\), and \(n\) is the number of distinct event types.
    
    \item We are specifically interested in the occurrence of core activities \(basis \in M\), where \(basis = e_j \in \Sigma\). Define \(basis\_count_i^{basis} = value_{ij}\) as the count of a specific, foundational event type within process instance \(i\), signifying the occurrence of a core activity essential for process validity.

    \item To evaluate adherence to the process norm, we identify the constraints \(C = \{(A, w_A), (D, w_D), (G, w_G)\}\) where \(A, D, G \in \Sigma\) are activities and \(w_A, w_D, w_G\) are their respective weights.

    \item For a trace \(\sigma_i\) with events \(E_{\sigma_i} = [A, D, A, F, C, \ldots]\), we check if all constraints are satisfied. If all activities \(A, D, G\) are present, the score for this layer \(S_i\) is 1.

    \item If any constraint is not satisfied, we add a penalty based on the weight of the missing activity. Let \(missing(\sigma_i, C)\) be the set of missing activities from \(C\) in \(\sigma_i\). The penalty for a trace \(\sigma_i\) is:
    \[
    penalty_i = \sum_{(a, w_a) \in C} (1 - \delta(a \in E_{\sigma_i})) \cdot w_a
    \]
    where \(\delta\) is an indicator function that is 1 if the activity \(a\) is present in \(E_{\sigma_i}\) and 0 otherwise.

    \item The adjusted score for Layer 1 is then:
    \[
    S_i = 1 - penalty_i
    \]

    \item The total number of event types is denoted by \(col\_count = n\).

    \item To measure how much a trace deviates from the norm with respect to the frequency of activities, we first extrapolate the frequency of the core activities to all activities. The optimal event distribution count, \(opt\_count_i\), is calculated as:
    \[
    opt\_count_i = col\_count \cdot basis\_count_i^{basis}
    \]
    assuming an ideal balance among all event types relative to the basis event.

    \item We then compute:
    \[
    diff\_count_i = |sum\_counts_i - opt\_count_i|
    \]
    This difference describes how much \(\sigma_i\) deviates from the ideal event distribution.
\end{itemize}

This scoring mechanism incorporates the additional layers of process norms with weights for each constraint:

\begin{itemize}
    \item \textbf{Layer 2: Sequential Directives:} Adjust \(S_i\) based on adherence to the mandatory sequence of events. Each pair \((a_1, a_2)\) has an associated weight \(w_{(a_1, a_2)}\). Formally, let:
    \[
    S_i = S_i - \sum_{(a_1, a_2) \in <_M} \alpha_{(a_1, a_2)} \cdot w_{(a_1, a_2)} \cdot (1 - \delta(\exists (e_1, e_2) \in E_{\sigma_i} \text{ where } \#_{\text{activity}}(e_1) = a_1 \text{ and } \#_{\text{activity}}(e_2) = a_2 \text{ and } e_1 <_{\sigma} e_2))
    \]
    where \(\alpha_{(a_1, a_2)}\) is a penalty factor, \(\delta\) is an indicator function that equals 1 if the condition is true and 0 otherwise.

    - For each pair \((a_1, a_2) \in <_M\), check if \(a_1\) eventually follows \(a_2\) in the trace \(\sigma_i\). If all constraints are satisfied, the score for this layer \(S_i\) is 1.
    - If any constraint is not satisfied, add a penalty based on the weight of the missing sequence. The penalty for a trace \(\sigma_i\) is calculated as shown in the formula above.

    \item \textbf{Layer 3: Equilibrium Standards:} Adjust \(S_i\) based on the balance of event occurrences. Each event \(h \in H\) should occur the same number of times, with an associated weight \(w_h\). Formally, let:
    \[
    S_i = S_i - \sum_{h \in H} \beta_h \cdot w_h \cdot \max(0, |\text{count}(h, \sigma_i) - \text{expected}(h)|)
    \]
    where \(\beta_h\) is a penalty factor, \(\text{expected}(h)\) is the expected count of event \(h\), and \(\text{count}(h, \sigma_i)\) is the actual count in trace \(\sigma_i\). The penalty is highest for events with the greatest deviation from the expected count.

    \item \textbf{Layer 4: Singularity Criteria:} Penalize instances with repeated occurrences of events that should be unique. Each unique event \(u\) has an associated weight \(w_u\). Formally, let:
    \[
    S_i = S_i - \sum_{u \in U} \gamma_u \cdot w_u \cdot \max(0, \text{count}(u, \sigma_i) - 1)
    \]
    where \(\gamma_u\) is a penalty factor, and \(U\) is the set of events that should be unique. The penalty increases with the number of extra occurrences.

    \item \textbf{Layer 5: Exclusion Guidelines:} Penalize instances that include unwished-for events. Each undesirable event \(a\) has an associated weight \(w_a\). Formally, let:
    \[
    S_i = S_i - \sum_{a \in A} \delta_a \cdot w_a \cdot \text{count}(a, \sigma_i)
    \]
    where \(\delta_a\) is a penalty factor, and \(A\) is the set of undesirable events. The penalty increases with the number of occurrences of the excluded events.
\end{itemize}

In these formulas:
- Each weight \(w\) is a value between 0 and 1, where 1 represents the highest penalty and 0 the lowest.
- The penalty factors \(\alpha_{(a_1, a_2)}\), \(\beta_h\), \(\gamma_u\), and \(\delta_a\) are scaled according to the corresponding weights, adjusting the impact of each constraint violation on the score \(S_i\).


This approach enables a nuanced analysis of process instances against a structured set of norms, facilitating targeted improvements in process execution and compliance.





==> Chapters_Singular/4_Evaluation.tex <==

\section{Evaluation and Results}

This section presents the evaluation results using the BPI 2019 dataset as a case study and reports on applying the method to industrial datasets. Our goal is to demonstrate the method's application on real-life data and provide feedback from an industrial case study, highlighting its effectiveness in identifying process inefficiencies and corresponding features.

\subsection{Evaluation of the BPI 2019 Dataset}
Our analysis utilizes the dataset provided by the BPI Challenge 2019, sourced from a multinational corporation in the coatings and paints sector in The Netherlands. This dataset provides a detailed view of the purchase order handling process across its 60 subsidiaries, with a specific focus on compliance \cite{vanDongen2019BPIDataset}.

\begin{figure}[ht]
  \centering
  \includegraphics[width=\columnwidth]{pictures/Scores_Distribution.png}
  \caption{Scores distribution in BPIC 2019 Dataset based on the defined Process Norm.} 
  \label{fig:ScoresDistributionBPIC2019}
\end{figure}

The BPIC 2019 dataset categorizes purchase order line items into four main process flows:
- **3-way matching with post-receipt invoicing**: Requires both GR-based and Goods Receipt flags to be true.
- **3-way matching with pre-receipt invoicing**: Invoices are issued before goods receipt but are blocked until receipt verification.
- **2-way matching without goods receipt**: Indicated by the absence of GR-based and Goods Receipt flags.
- **Consignment**: Identified by a true GR indicator but a false GR IV flag.

Using the method outlined in Definition \ref{def:process_norm} and Section \ref{sec_method}, we defined a process norm based on our comprehensive understanding of procurement operations and insights from the BPIC 2019 description and reports. Essential activities for every procurement cycle, such as "Create Purchase Order Item" and "Record Goods Receipt," were included in the \textit{Foundational Protocols Layer}. Contrarily, activities like "Change Price" and "Change Vendor" were identified as counterproductive due to their manual nature, introducing inefficiencies, and were thus added to the \textit{Exclusion Guidelines Layer} constraints.

\begin{figure}[ht]
  \centering
  \includegraphics[width=\columnwidth]{pictures/Views_Layer_Importance.png}
  \caption{Scores for process instances based on different Process Views.} 
  \label{fig:InstanceScores}
\end{figure}

Figure \ref{fig:ScoresDistributionBPIC2019} shows the distribution of scores for different layers. This distribution suggests that different types of process flows may require different types of constraints. Additionally, depending on the business objective, scores can vary significantly. Figure \ref{fig:InstanceScores} illustrates an example of a singular process instance score for different process views. In this case, we observe high process scores for the \textit{Foundational Layer} from the \textit{Standardization Process View} perspective, while the score for the \textit{Process Cost View} perspective is much lower. By aggregating scores for the whole trace or over a particular set of traces, process analysts can identify areas with the highest inefficiencies, such as process costs, that should be further analyzed, especially in the \textit{Foundational Layer} scores.


The analyst can see the score distribution for a particular dataset feature. The result of such an analysis is depicted in Figure \ref{fig:Score_Dist_Feature}. The color shows at first glance that for this feature of data, the Logistic category can be interesting.

\begin{figure}[ht]
  \centering
  \includegraphics[width=\columnwidth]{pictures/Score_Distribution_Feature.png}
  \caption{Scores Distribution for Process Cost View aggregated over all traces.} 
  \label{fig:Score_Dist_Feature}
\end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[width=\columnwidth]{pictures/Logistic_Heatmap.png}
  \caption{Scores Distribution for Data from previous dataset with filter only on those with low performing scores.} 
  \label{fig:Score_Logistic}
\end{figure}
Based on results depicted in \ref{fig:Score_Dist_Feature} we filtered for only those with lowest performers categories. After that we found the feature of data that could describe low performance and analyzed it again. As a result we identified particular types of low performers such as \textit{Road Packed}, \textit{Sea} and \textit{Warehousing} which performed exceptionally poorly. We could also discover that areas of \textit{Exclusion Layer}, \textit{Equilibrium Layer} and \textit{Singularity Layer} showed poorest score, which could suggest that in those areas a lot of manual changes and rework was taking place. This could be identified as root cause for the problems in this particular areas. Apart from that we could also discover poor performance in \textit{Service} Category and interesting patterns of particular Vendors. 




\subsection{Comparison between BPIC 2019 Challenge Papers and WISE Reporting}

\begin{figure}[ht]
  \centering
  \includegraphics[width=\columnwidth]{pictures/ChatGPT4_Analyst.png}
  \caption{Part of LLM \textit{ChatGPT4} analysis suggesting additional areas of interest and further steps.} 
  \label{fig:ChatGPT}
\end{figure}

The WISE Method not only facilitates various data dicing, slicing, and drilling-down techniques combined with statistical and machine learning methodologies but also enables the automated detection of features that can be interesting for process analysts. Our automated workflow allows for utilizing Large Language Models in the role of the analyst. This can be used to support Process Norm creation, add weights to different layers, analyze singular figures, or even create whole reports with management summaries and detailed project plans for process improvement in the form of PDF files.

\begin{figure}[ht]
  \centering
  \includegraphics[width=\columnwidth]{pictures/Shared_Words_Barplot.png}
  \caption{The most common shared words between BPIC 2019 Challenge Papers and automated Report.} 
  \label{fig:SharedWords}
\end{figure}
For a more comprehensive analysis, we created a detailed report (74 pages) for the BPIC 2019 dataset, using Chat-GPT 4o as analyst, and compared it with all 15 papers presented as part of the BPIC 2019 challenge. 

Figure \ref{fig:ChatGPT} illustrates an excerpt from this automated analysis, highlighting categories with high and low performers, and suggesting further detailed investigations. We assessed how the automated report differed from the manually analyzed results in the BPIC 2019 challenge papers. 

Figure \ref{fig:SharedWords} shows the words shared between the challenge papers and the automated report. Some areas, such as packaging or marketing, are clearly identified as important in both the challenge papers and the WISE Report, as indicated in the figure. Additionally, most analyses described logistics as one of the areas requiring further examination. However, the challenge papers generally did not delve deeper or analyze in detail different correlations and impactful data features, such as specific employees or vendors. The WISE Analysis provided these findings almost instantly.

Overall, the challenge papers were more focused on process flow attributes, whereas the WISE Report identified the most substantial areas for improvement, offering detailed proposals. These detailed findings, compounded with different layers representing various types of challenges, enabled the formulation of hypotheses about root causes, such as the incorrect order of mandatory activities or rework.




\subsection{Industrial Case Evaluation}

The method was evaluated in an industrial setting within a real estate company managing a substantial property portfolio. This evaluation was part of a procurement improvement initiative aimed at enhancing the transparency and standardization of the procurement process, which is crucial for effective property management.

The current procurement process is characterized by significant complexity and variability. The company deals with over 100,000 different materials from more than 20,000 suppliers, resulting in over 58,000 process variants, with the top 10 accounting for only 8\% of all instances. This high variability complicates the identification of standard practices and optimization of the procurement process. While the analysis revealed several bottlenecks and inefficiencies, it struggled to pinpoint specific issues due to the overwhelming data and unclear patterns.

The optimization project faced several challenges:
\begin{enumerate}
    \item \textbf{Supply Chain Variability}: The vast number of suppliers introduces variability in quality, reliability, and terms of supply, leading to inconsistencies in procurement practices and challenges in maintaining standardization.
    \item \textbf{Materials Management Complexity}: Managing over 100,000 different materials adds substantial complexity, as different materials may require varied handling and procurement strategies.
    \item \textbf{Quality Assurance Issues}: Ensuring that all ordered materials meet specified quality standards is critical. Robust quality assurance processes are essential to prevent the use of substandard materials, which can cause maintenance failures and increased costs.
\end{enumerate}

Addressing these challenges, the project aimed to enhance transparency and standardization in the procurement process. One main objective was to identify drivers of variability, determining whether variability is driven by material properties, specific suppliers, or inherent process complexities.

\subsubsection{Implementation of Scoring Mechanism}

The business objective of decreasing supply chain variability was defined as part of a broader strategy through top management. Grounded on this goal, we conducted internal procurement workshops to develop a matrix that evaluates the norms and the significance of individual problems identified within the process. Figure \ref{fig:WISEMethod} depicts different phases of the project and the parties responsible for various stages of execution.

\begin{figure}[ht]
  \centering
  \includegraphics[width=\columnwidth]{pictures/Method.png}
  \caption{Phases of the process improvement project supported by the WISE Methodology.}
  \label{fig:WISEMethod}
\end{figure}

Domain experts and process analysts were invited to the project, ensuring the Process Norm was built with a perspective of process improvement towards the defined business objective. Discussions focused on actionable areas within the company's control.

Based on the Definition of the Process Norm defined in \ref{def:process_norm}, we defined the constraints and weights for all layers. The following are excerpts of findings for particular layers for the specific business objective:

\begin{itemize}
    \item \textbf{Sequential Directives}: Simplified but included variants addressing processes under a Framework Agreement, eliminating the need for steps like additional approvals.
    \item \textbf{Equilibrium Standards}: Critical for process instance variability, verifying quantities, quality checks upon goods receipt, and financial consistency from purchase requisition to invoice payment.
    \item \textbf{Singularity Criteria}: Aimed to eliminate repeated releases and checks, identified as significant contributors to increased process time and variability.
    \item \textbf{Exclusion Guidelines}: Identified costly and detrimental tasks to process automation, including unnecessary communications and changes to critical elements such as prices, quantities, currency, or key fields in purchase orders.
\end{itemize}

\subsubsection{Results of Procurement Optimization Project}

The comparative analysis and reports identified areas of interest, facilitated by pre- and post-WISE analysis workshops that improved communication between process improvement specialists and domain experts. Figures \ref{fig:AllNorms1} and \ref{fig:AllNorms2} depict partial anonymized results.
\begin{figure}[ht]
  \centering
  \includegraphics[width=\columnwidth]{pictures/All_Norms_Properties.png}
  \caption{Example of Summarized Norms Scoring grouped by different locations.}
  \label{fig:AllNorms1}
\end{figure}
Figure \ref{fig:AllNorms1} synthesizes a detailed assessment of scoring norms across properties, grouped by geographic location. The boxplot segments,darker color meaning biggest volume of orders, correspond to scores calculated by WISE algorithms.

\begin{figure}[ht]
  \centering
  \includegraphics[width=\columnwidth]{pictures/All_Norms_Properties_MaterialGroup.png}
  \caption{Example of Summarized Norms Scoring based on material group.}
  \label{fig:AllNorms2}
\end{figure}

The variability in compliance is visually evident, with the interquartile ranges (IQRs) varying in width across the properties. Properties like 'China 2' and 'Greece' exhibit high adherence, indicated by narrow boxplots, while 'Switzerland' shows less consistency. The color differentiation indicates the count of ordered positions by location, illustrating that a higher volume of orders does not directly correlate with lower process scores.

Figure \ref{fig:AllNorms2} provides an analysis based on the aggregated scores for each material group. In contrast to Figure \ref{fig:AllNorms1}, which showed a more homogeneous distribution of scores, Figure \ref{fig:AllNorms2} reveals pronounced variability among different material groups, with security services, maintenance, and utilities emerging as areas of concern due to their problematic scores.

The analysis efficiently pinpointed significant challenges within various categories. Subsequent investigations revealed specific correlations, such as suppliers deviating from standard procedures or equipment requiring additional user training for departmental staff.

Overall, the project successfully highlighted sectors where improvements are feasible. Recommendations include renegotiating contracts with certain suppliers, modifying material templates for select categories, and implementing specialized documentation or training for specific equipment. These strategic measures are anticipated to yield substantive improvements in the procurement process.



==> Chapters_Singular/5_Conclusion.tex <==
\section{Conclusion}

This study demonstrates the effectiveness of the WISE Methodology in identifying and addressing process inefficiencies within complex procurement environments. By defining process norms and applying a structured scoring mechanism, the methodology highlights areas of variability, inefficiency, and potential improvement.

The evaluation of the BPI 2019 dataset revealed that different types of process flows require distinct constraints and norms, enabling more precise tailoring of process improvement initiatives. The detailed scoring of process instances provides a comprehensive view of process performance and areas for enhancement.

The industrial case study underscores the practical applicability of the WISE Methodology. Despite the complexity and variability of the procurement process, the method successfully identified critical activities and provided optimization recommendations that can significantly improve procurement efficiency and standardization.

While leveraging Large Language Models (LLMs) for automated analysis and report generation offers innovative solutions, it is essential to have a Human in the Loop. Automated reports must be validated against the real experience of domain experts to ensure accuracy and relevance.

Future steps include creating a correlation matrix between different layers and their mapping to specific challenges, such as low sequential layer scores indicating potential issues in particular areas. Additionally, refining the architecture for automated report generation and adding features to support cooperation between analysts and LLMs will further enhance the effectiveness of the WISE Methodology.

In summary, the WISE Methodology is a valuable tool for organizations seeking to enhance their procurement processes, offering a structured approach to process improvement supported by advanced analytical capabilities.

